Sim and Real: Better Together

Simulation is used extensively in autonomous systems, particularly in robotic manipulation. By far, the most common approach is to train a controller in simulation, and then use it as an initial starting point for the real system. We demonstrate how to learn simultaneously from both simulation and interaction with the real environment. We propose an algorithm for balancing the large number of samples from the high throughput but less accurate simulation and the low-throughput, high-fidelity and costly samples from the real environment. We achieve that by maintaining a replay buffer for each environment the agent interacts with. We analyze such multi-environment interaction theoretically, and provide convergence properties, through a novel theoretical replay buffer analysis. We demonstrate the efficacy of our method on a sim-to-real environment.

==> bounds_sim_real_critic.tex <==
\subsection{Bounds on sim to real}
Analysis based on \cite{perkins2002convergent}.

First, we define $P_{1}^\pi$ to be the $(|\mathcal{S}| \cdot |\mathcal{A}|)  \times (|\mathcal{S}| \cdot |\mathcal{A}|)  $ matrix whose entries correspond to the probabilities that one state-action pair follows another when the agent behaves according to $\pi$ in MDP $M_{1}$. That is, the element on the $(s,a)^\text{th}$ row and $(s',a')^\text{th}$ column of $P_{1}^\pi$ is $p_{1}(s'|s,a) \pi (a'|s')$. $P_{1}^\pi$  can be viewed as the stochastic transition matrix of a Markov chain over state-action pairs. Note that $p_{1}, p_{2} \in \mathbb{R}^{|\mathcal{S}| \cdot |\mathcal{A}| \cdot |\mathcal{S}|} $. A similar definition is for $P_{2}^\pi$. Note that $p_{1}, p_{2} \in \mathbb{R}^{|\mathcal{S}| \cdot |\mathcal{A}| \cdot |\mathcal{S}|} $.

\begin{lemma}
\label{lemma:p_bound}
There exists $c_p$ such that for all $p_{1}$, $p_{2}$, $\|P_{1}^\pi - P_{2}^\pi \|_2 \le c_p \| p_{1} - p_{2}\|_2$.
\end{lemma}

{\bf proof}: Let $p_{1}$, $p_{2}$ be fixed, and let $i = (s,a)$ and $j=(s',a')$. Recall that $\pi (a'|s') \le 1$ for all $s, a$. Then:
\begin{equation}
    \begin{split}
        | P_{1_{i,j}}^\pi - P_{2_{i,j}}^\pi| &= \big| \pi (a'|s') \big( p_{1}(s'|s,a)  - p_{2}(s'|s,a) \big) \big| \\
        & \le \big| p_{1}(s'|s,a)  - p_{2}(s'|s,a)  \big| \\
        & \le \max_{s,a, s'} \big| p_{1}(s'|s,a)  - p_{2}(s'|s,a)  \big| \\
        &  = \| p_{1}  - p_{2}  \|_\infty \\
        &  \le \| p_{1}  - p_{2}  \|_2 
    \end{split}
\end{equation}

For any $l$-by-$l$ matrices A and B whose elements different in absolute value by at most $\epsilon$, $\| A - B\| \le \sqrt{l}\epsilon$. Thus 
\[\|P_{1}^\pi - P_{2}^\pi \|_2 \le \sqrt{|\mathcal{S}| \cdot |\mathcal{A}|} \| p_{1}  - p_{2}  \|_2 \le \sqrt{|\mathcal{S}| \cdot |\mathcal{A}|} \cdot \epsilon_p \]
That is, $c_p = \sqrt{|\mathcal{S}| \cdot |\mathcal{A}|}$

\sd{TODO: decide whether assume: $\max_{s,a, s'} \big| p_{1}(s'|s,a)  - p_{2}(s'|s,a)  \big| \le \epsilon_p $ or $\| p_{1}  - p_{2}  \|_2 \le \epsilon_p$ }

\begin{lemma}
\label{lemma:mu_bound}
There exists $c_\mu^1$ and $c_\mu^2$ such that for all $p_{1}$, $p_{2}$, $ \|\mu_{1}^\pi - \mu_{2}^\pi\|_2 \le c_\mu^1 \| p_{1} - p_{2}\|_2$ and $\|\mu_{2}^\pi - \mu_{1}^\pi\|_2 \le c_\mu^2 \| p_{2} - p_{1}\|_2$
\end{lemma}

\begin{proof}
Under Assumption \ref{ass:aperiodic}, fixing a policy, $\pi$, induces an irreducible, aperiodic Markov chain over $\mathcal{S}$. Let $d_{1}^\pi(s) > 0$ 
denote the stationary probability of state $s$ under policy $\pi$ and MDP $M_{1}$. We define $\mu_{1}^\pi$  to be
the length $|\mathcal{S}| \cdot |\mathcal{A}|$ vector whose $(s,a)^{\text{th}}$ element is $d_{1}^\pi(s) \pi(a|s)$. Note that the elements of $\mu_{1}^\pi$ sum to one. If  $ \pi(a|s) > 0$	for all $s$ and $a$, then all elements of $\mu_{1}^\pi$ are positive and it is easily verified that $\mu_{1}^\pi$ is the unique stationary distribution of the irreducible, aperiodic
Markov chain over state-action pairs with transition matrix $P_{1}^\pi$. 

\citet{seneta1991sensitivity}
showed that for any two irreducible  aperiodic Markov chains with transition matrices $P_1$ and $P_2$ and stationary distributions $\mu_1$ and $\mu_2$: 
on a state set with $l$ elements:
\[\| \mu_1 - \mu_2\|_1 \le \frac{l}{|1 - \lambda_1|} \| P_1 - P_2\|_{\infty}\]
where $\lambda_1$ is the largest eigenvalue of $P_1$ with modulus strictly less than one. We denote by $\lambda_{1}^{\text{max}}$ the largest eigenvalue of $P_{1}^\pi$ with modulus strictly less than one. Then,
\begin{equation}
    \begin{split}
        \|\mu_{1}^\pi - \mu_{2}^\pi\|_2 & \le \|\mu_{1}^\pi - \mu_{2}^\pi\|_1 \\
        & \le \frac{|\mathcal{S}| \cdot |\mathcal{A}|}{|1 - \lambda_{1}^{\text{max}}|} \| P_{1}^\pi - P_{2}^\pi\|_{\infty} \\
        & \le \frac{|\mathcal{S}| \cdot |\mathcal{A}|}{|1 - \lambda_{1}^{\text{max}}|} \| P_{1}^\pi - P_{2}^\pi\|_2 \\
        & \le \frac{|\mathcal{S}| \cdot |\mathcal{A}|}{|1 - \lambda_{1}^{\text{max}}|} c_p \| p_{1} - p_{2}\|_2 \\
         & = c_\mu^1 \| p_{1} - p_{2}\|_2 \\
    \end{split}
\end{equation}
where $c_\mu^1 = \frac{|\mathcal{S}| \cdot |\mathcal{A}|}{|1 - \lambda_{1}^{\text{max}}|} \cdot c_p $. Similarly, we can prove $\|\mu_{2}^\pi - \mu_{1}^\pi\|_2 \le c_\mu^2 \| p_{2} - p_{1}\|_2$ with $c_\mu^2 = \frac{|\mathcal{S}| \cdot |\mathcal{A}|}{|1 - \lambda_{2}^{\text{max}}|} \cdot c_p $.

\end{proof}

We define $D^{\pi}_{1}$ to be the matrix whose diagonal is $\mu_{1}^\pi$ . Then:
\[ \| D^{\pi}_1 - D^{\pi}_2 \| \le  \|\mu_{1}^\pi - \mu_{2}^\pi\|_2\]



We want to bound the following term $\| \bold{v}_1 - \bold{v}_2 \|$. Let us assume both sim and real satisfy the following equations:
\begin{equation*}
    \begin{split}
        A_1 \bold{v}_1 &= b_1 \\
        A_2  \bold{v}_2 &= b_2 \\
    \end{split}
\end{equation*}
where:
\begin{equation*}
    \begin{split}
        A_1 &= \boldsymbol{\Phi}^\top D_1 (P_1 - I) \boldsymbol{\Phi} \\
        A_2 &= \boldsymbol{\Phi}^\top D_2 (P_2 - I) \boldsymbol{\Phi} \\
        b_1 & = \boldsymbol{\Phi}^\top D_1 \bold{r}_1 \\
        b_2 & = \boldsymbol{\Phi}^\top D_2 \bold{r}_2
    \end{split}
\end{equation*}
Now, let's subtract these two equations. The following equations are equal:
\begin{equation}
    \begin{split}
        A_1 \bold{v}_1 - A_2 \bold{v}_2 &= b_1 - b_2\\
        A_1 \bold{v}_1 - A_1 \bold{v}_2 + A_1\bold{v}_2 - A_2 \bold{v}_2 &= b_1 - b_2\\
        A_1( \bold{v}_1 -  \bold{v}_2)  &= b_1 - b_2 -( A_1 - A_2)\bold{v}_2 \\
        ( \bold{v}_1 -  \bold{v}_2)  &= A_1^{-1}(b_1 - b_2) -A_1^{-1}( A_1 - A_2)\bold{v}_2 \\
        \| \bold{v}_1 -  \bold{v}_2\|  &= \|A_1^{-1}(b_1 - b_2) -A_1^{-1}( A_1 - A_2)\bold{v}_2 \| \\
        \| \bold{v}_1 -  \bold{v}_2\|  & \le \|A_1^{-1}\| \big(  \|b_1 - b_2\| +  \| A_1 - A_2\| \cdot \|\bold{v}_2 \| \big) \\
    \end{split}
\end{equation}
Now we look at each term separately:
\begin{equation*}
    \begin{split}
    \| b_1 - b_2\| & =  \| \boldsymbol{\Phi}^\top D_1 \bold{r}_1  - \boldsymbol{\Phi}^\top D_2 \bold{r}_2\| \\
    & = \| \boldsymbol{\Phi}^\top \left( D_1 \bold{r}_1  -  D_2 \bold{r}_2 \right)\| \\
    & = \| \boldsymbol{\Phi}^\top \left( D_1 \bold{r}_1 +D_1 \bold{r}_2 - D_1 \bold{r}_2  -  D_2 \bold{r}_2 \right)\| \\
    & = \| \boldsymbol{\Phi}^\top \big( D_1 (\bold{r}_1 - \bold{r}_2) + (D_1 - D_2) \bold{r}_2 \big)\| \\
    & \le \| \boldsymbol{\Phi}^\top \| \Big( \| D_1 \| \|\bold{r}_1 - \bold{r}_2\| +  \|D_1 - D_2\| \|\bold{r}_2\| \Big)\\
    &\stackrel{1}{\le}  \| \boldsymbol{\Phi}^\top \| \Big( \|\bold{r}_1 - \bold{r}_2\| +  c_\mu \|p_1 - p_2\|_2 \|\bold{r}_2\| \Big)
    \end{split}
\end{equation*}
where in inequality (1) we used Lemma \ref{lemma:mu_bound} and $\| D_1 \| \le 1$.

\begin{equation*}
    \begin{split}
    \| A_1 - A_2\| & =  \| \boldsymbol{\Phi}^\top D_1 (P_1 - I) \boldsymbol{\Phi} - \boldsymbol{\Phi}^\top D_2 (P_2 - I) \boldsymbol{\Phi}\| \\
    & = \| \boldsymbol{\Phi}^\top \Big( D_1 (P_1 - I) -  D_2 (P_2 - I) \Big) \boldsymbol{\Phi}\| \\
    & = \| \boldsymbol{\Phi}^\top \Big( D_1 P_1 - D_1 -  D_2 P_2 + D_2 + D_1 P_2 - D_1 P_2  \Big) \boldsymbol{\Phi}\| \\
    & = \| \boldsymbol{\Phi}^\top \Big( D_1( P_1 - P_2) + (D_1 - D_2) (P_2 - I) \Big) \boldsymbol{\Phi}\| \\
    & \le \| \boldsymbol{\Phi}^\top \| \Big(\|  D_1( P_1 - P_2) + (D_1 - D_2) (P_2 - I)  \| \Big) \|\boldsymbol{\Phi}\| \\
    & \le \| \boldsymbol{\Phi}^\top \| \Big( \|  D_1\| \| P_1 - P_2 \| + \|D_1 - D_2\| \|P_2\| +  \|D_2 - D_1\|  \Big)\|\boldsymbol{\Phi}\| \\
    &\stackrel{1}{\le} \| \boldsymbol{\Phi}^\top \| \Big(c_p \| p_1 - p_2 \| + c_\mu^1 \| p_1 - p_2 \|  +  c_\mu^2 \|p_2 - p_1\|  \Big)\|\boldsymbol{\Phi}\| \\
    \end{split}
\end{equation*}

where in inequality (1) we used Lemma \ref{lemma:p_bound}, Lemma \ref{lemma:mu_bound}, $\| P_2\| = 1$ and $\| D_1 \| \le 1$.
  









==> continuous_stationary.tex <==
\subsection{Continuity of eigenvectors}
We first state a result from \cite{bhatia2013matrix} regarding the continuity of eigenvalus.
\begin{lemma}[Continuity of Eigenvalues. Corollary VI.1.6 in \cite{bhatia2013matrix}]
\label{lemma:beta_continuity}
Let $\beta \rightarrow {\bf P}(\beta)$ be a continuous map from an interval I into the space of $|\mathcal{S}| \times |\mathcal{S}|$ matrices. Then, there exist continuous functions $\lambda_1(\beta), \lambda_2(\beta), \ldots \lambda_{|\mathcal{S}|}(\beta)$ that, for each $\beta \in I$, are the eigenvalues of ${\bf P}(\beta)$.

\end{lemma}
Let ${\bf x}$ be a left eigenvector of a stochastic matrix ${\bf P} \in \mathbb{R}^{n \times n}$ corresponding to eigenvalue $\lambda$, then:
\[{\bf x}^\top {\bf P} = \lambda {\bf x}^\top\]
\[{\bf x}^\top ({\bf P} - \lambda {\bf I}) = {\bf 0}\]

Since ${\bf P}$ is stochastic, it has a left eigenvector $\boldsymbol{\mu}$ corresponding to eigenvalue $\lambda=1$, where $\boldsymbol{\mu}$ is the stationary distribution of ${\bf P}$, then:
\[\boldsymbol{\mu}^\top ({\bf P} - {\bf I}) = {\bf 0}\] 
From the rank-nullity theorem:
\[n = rank({\bf P - I}) + null({\bf P - I})\]
\[null({\bf P - I}) = dim\big(ker({\bf P - I}) \big)\]
\[dim\big(ker({\bf P - I}) \big) = \big| \{ {\bf y} \ | \ ({\bf P - I}){\bf y} = 0 \cdot {\bf y} = {\bf 0}\}\big|\]

The kernel of ${\bf P - I}$ is precisely the eigenspace corresponding to eigenvalue 0.  The matrix ${\bf P - I}$ has eigenvalue of 0 with multipicity 1, then 
\[dim\big(ker({\bf P - I}) \big) = 1\]
\[\Rightarrow rank({\bf P - I}) = n - 1\]
This means we have a linear system with $n-1$ equations.$ ({\bf P - I})$ is not invertible and there are infinite number of solutions. However, if we add the constraint of $\|\boldsymbol{\mu}\|=1$ (the stationary distribution is a vector of probabilities summing to 1), we add another equation to the system and now we have a single solution. Thus, we can view $\boldsymbol{\mu}$ as a function of ${\bf P}$ and $\lambda$ with only one image to each input. Since ${\bf P}$ is continuous in $\beta$
\[{\bf P} = \beta {\bf P}_1 + (1-\beta)  {\bf P}_2\]
and since the eigenvalue $\lambda$ is continuous according to Lemma \ref{lemma:beta_continuity}, then $\boldsymbol{\mu}$ is a composition of continuous functions, thus it is continuous. 


==> distribution_RB.tex <==
\subsection{Distribution Of the states in the RB}
\begin{lemma}
Suppose we have a RB with $N$ samples. Let us assume that the current-state $s$ for each samples in the replay buffer correspond to parameters $\theta_{\tau-N+1},\ldots,\theta_{\theta}$, respectively. Let $P_{\theta_i}$ be a matrix with elements $P_{\theta_i}^{(mn)}$ in row $n$ and column $m$
\begin{equation*}
    P_{\theta_\tau}^{(mn)} \triangleq P(s'=m| s=n) = \sum_{a \in \mathcal{A}} P(s'|s,a) \pi_{\theta_{\tau}} (a|s).
\end{equation*}
We denote by $\rho_\tau$ the state distribution at time $\tau$, which satisfies
\begin{align*}
    \rho_{\tau+1}^\top &= \rho_{\tau}^\top P_{\theta_{\tau}}\\
    \Rightarrow \rho_{\tau+2}^\top &= \rho_{\tau}^\top P_{\theta_{\tau}} P_{\theta_{\tau+1}}\\
\end{align*}

We denote with $\bold{s}$ and $\bold{s}'$ vectors correspond to distribution of $s$ and $s'$, respectively. \sd{Shouldn't we denote it as $\bold{s}_{\tau}$?} \sd{We need a different definitions for $\bold{s}$ and $\rho_\tau$ since we called them both "state distribution" and the difference is not clear}%In addition, we assume the state distribution at time $\tau-N$ is the stationary distribution $\mu_{\tau-N}$. 
Then, \\
\noindent \textbf{1.} The vector $\bold{s}$ is
\begin{equation}
    \bold{s}^\top \sim \frac{1}{N} \sum_{t=\tau-N+1}^\tau \rho_{\tau-N}^\top
    \prod_{i=\tau-N+1}^{t} P_{\theta_i}.
\end{equation}
\noindent \textbf{2.} The distribution of state $s' \in \mathcal{S}$ in the RB is
\begin{equation}
    \bold{s}'^\top \sim \frac{1}{N} \sum_{t=\tau-N+1}^\tau \rho_{\tau-N}^\top
    \prod_{i=\tau-N+1}^{t+1} P_{\theta_i}.
\end{equation}
\noindent \textbf{3.} The distribution of the consecutive states $(s, s')$ where $s, s'\in \mathcal{S}$ in the RB are expressed with the matrix $\bold{S} \triangleq\bold{s} \bold{s}'^\top$ where the row correspond to $s$ and the column correspond to $s'$.
\end{lemma}


==> expectation_TD_Linear_FA.tex <==
\subsection{Single environment}
\begin{lemma}
Let us assume in time $\tau-N$ the distribution is $\rho_{\tau-N}$. The following holds
\begin{equation*}
\begin{split}
    \mathbb{E}_{\tilde{\mathcal{O}} \sim \text{RB}}
    \left[
    \delta(\tilde{\mathcal{O}}) \phi (\tilde s)
    \right]
    & =
    \Phi^{\top} \left(\frac{1}{N} \sum_{i=1}^N S_{\theta_{\tau-i}} (P_{\theta_{\tau-i}} - I) \right)\Phi v + \Phi^{\top} \left(\frac{1}{N} \sum_{i=1}^N  S_{\theta_{\tau-i}}\right) (r-\eta)\\
    \end{split}
\end{equation*}
where 
\begin{equation*}
    S_{\theta_{\tau-i}} = \textrm{diag}
    \left(
    \mu_{\tau-N}
    \prod_{j=\tau-N}^{\tau-i}P_{\theta_{j}}
    \right).
\end{equation*}
\end{lemma}

\begin{proof}

\end{proof}

==> experiment_panda_robot.tex <==
\subsection{Robots Experimental Setup}
% I've based this description (only the structure) on the QTOpt 
\subsubsection{General Setup}

Our setup consists of two parts: The robotics arm and the simulator. For the real robot setup, we use a Franka Emika robotic arm (\citealp{franka_emika}; called "Panda") with 7 degrees of freedom (DPF). For the perception, an Intel RealSense 415 camera is mounted from an angular position (see Figure \ref{fig:franka_setup_photo}) and connected to the robot. For the simulated part we use MuJoCo \citep{todorov2012mujoco} as the physics engine, and a version of the Fetch Push environment \cite{plappert2018multi}  that was adapted to resemble our robot setup.  The box and ball setup are similar both in the reality and simulation in terms of size, weight and colors. Further experiment details are described in the supplementary material. 
%We use the research version of the arm which allows its user to have a direct control and the possibility to program the robot and interface the robot with external sensors.

We denote by $q_r$ the samples rate of the robot, and with $q_s$ the sample rate of the simulation. In our setup, we found that the rate between simulation and reality is $\nu_s/\nu_r \approx 85$.





\subsubsection{State Space and Perception Setup}
The robot's task is push a cube from its current position to a goal position. An RGB camera (D415 RealSense, Intel) was used to provide a perception of the cube position. We used distinct colors to localize the cube in the RGB image. At the beginning of each episode, the goal position is sampled. Both sim and real share the same state space with dimension 12: $3$ for the gripper position $3$ for the cube position in $3$ for the relative distance between the gripper and the cube and $3$ for the gripper translation velocity. In addition we added to the state representation the goal position, to support the HER environment \cite{andrychowicz2017hindsight}. 
The action specify the desired gripper poistion at the next time step (dimension $4$). Both the state space and the action space are continuous.



\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.75\columnwidth]{pictures/robot_panda_1.jpg}}
\caption{Setup of the robotic arm. The panda robot is positioned on the table while  the RealSense camera is positioned in the right upper corner. The cube  is on the table.}
\label{fig:franka_setup_photo}
\end{center}
\vskip -0.2in
\end{figure}


\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.75\columnwidth]{pictures/fetch_box_success_2.jpg}}
\caption{The task of the robot is to push the box (red) to a goal position (blue).}
\label{fig:ball_and_goal}
\end{center}
\vskip -0.2in
\end{figure}


\subsection{Robots Experimental Results}
We ran experiments on a single robot and a single simulation. In figure \ref{fig:sim_and_real_example} we show the setup in MuJoCo simulation and on real robot. We set the ratio for learning from the two replay buffers to be $\beta_r/\beta_s=1$. The throughput of samples from simulation is roughly 85 times higher then the throughput of samples from the robot. 

We chose this experiment since to the best of our knowledge none of existing simulations can really model accurately enough the dynamics of a ball rolling inside the box. But nevertheless, many aspects of the dynamics are still captured in simulation (e.g., direction of the moving ball in response to the gripper pushing it).




\subsection{Supplementary}
\subsubsection{Hardware Setup}
The setup involved two workstations: a CPU Intel i7 workstation that functioned as the Panda robot and RealSense camera controllers, and a CPU i7 workstation with two 2080Ti GPUs for running the simulation and the coordinator agent. All parts were connected using a 1Gbit network. \sd{Check details}

\subsubsection{Software Stack}
For controlling the robot, we use robotic operating system (ROS Melodic; \citealp{ros_melodic}). We use two controllers interchangeably: Impedance Control \citep{lynch2017modern} for small and delicate manipulations, and Moveit \citep{chitta2012moveit} for motion control of larger pose changes. For controlling the simulator we used Mujoco. For communication between sim and real we used the Redis framework \citep{carlson2013redis}.
\subsubsection{Action Space}
The action corresponds to the delta step of the gripper position in each one of the 3D Cartesian coordinates. %The learner was allowed to choose any rotation within a safe working range, so in many cases the object does not move at all.

==> finite_analysis.tex <==
\section{Finite sample analysis}
\sd{In work}
This analysis is based on \cite{wu2020finite} and \cite{zou2019finite}.

%Let $\mu_{\theta,Y}$ be the the stationary distribution of the Markov process $\{Y_{\tau}\}_{\tau \ge 0}$ induced by policy $\pi_\theta$, that is:
%\[\mu_{\theta,Y}^\top = \mu_{\theta,Y}^\top P(Y_{\tau+1} | Y_\tau).\]
In this section we assume we have $K=2$ environments. $k=1$ is the real environment and $k=2$ is the sim environment.



%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}{Uniform ergodicity.}
\label{ass:uniform_ergodic}
 For a fixed $\theta$, denote $\mu_1(\theta)(\cdot)$ as the stationary distribution
induced by the policy $\pi_\theta(\cdot|s)$ and the transition probability measure $P_1(\cdot|s,a)$ ("$P_{\text{real}}$"). Consider a Markov chain generated by the rule $a_t \sim \pi_\theta(\cdot|s_t)$, $s_{t+1} \sim P_1(\cdot|s_t,a_t) $. 
Let $d_1(t)$ denote the state distribution of the Markov chain after $t$ time-steps. Then, there exist constants $m > 0$ and $\kappa \in (0, 1)$ such that:
    \[\| d_1(t) - \mu_1(\theta) \| \le m \kappa^t \ \forall \ t \ge 0 \]
    where $\|\cdot\|$ denote the total variation norm on $\mathcal{S}$. 
\end{assumption}

\begin{lemma}
\label{lemma:dvt3}
Under assumption \ref{ass:uniform_ergodic}, 
\begin{align*}
    \| \rho(t) - d_1(t)\| \le \begin{cases} t (1 - q_1) \|  {\bf P}_2 - {\bf P}_{1}  \| & t < \hat{t} \\ 
    \Big( \hat{t} + m \frac{ \kappa^{\hat{t} } - \kappa^{t} }{1 - \kappa}\Big) \cdot (1 - q_1) \|  {\bf P}_2 - {\bf P}_1  \|  & t \ge \hat{t}
    \end{cases}
\end{align*}
where $ \hat{t} = \lceil{\log_\kappa m^{-1}}\rceil $.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:dvt3}]
%The proof is based on Theorem 7.5 in \cite{montenegro2006mathematical} and Theorem 3.1 in  \cite{mitrophanov2005sensitivity} 
For some initial state distribution $\rho_0$, Let $\rho(t)$ be the state distribution of the mixed Markov process $Y_\tau$, after $t$ time steps, $ \rho(t)^\top = \rho(0)^\top \prod_{t'=1}^{t-1} P_{t'}$. Note that $\rho(t)$ corresponds to the transition matrix $P$, which in our setup satisfies $P = q_1P_1 + q_2P_2$ for $K=2$. Now, consider another Markov chain generated by the rule $a_t \sim \pi_\theta(\cdot|s_t)$, $s_{t+1} \sim P_1(\cdot|s_t,a_t)$. 
Let $d_1(t)$ denote the state distribution of the Markov chain after $t$ time-steps.

We now bound the total variation distance between these two state distributions. According to Theorem 3.1 in  \cite{mitrophanov2005sensitivity},
\begin{align*}
    \| \rho(t) - d_1(t)\| \le \begin{cases} \| \rho(0) - d_1(0) \| + t \|  {\bf P} - {\bf P}_{1}  \| & t < \hat{t} \\ 
    m \kappa^t \| \rho(0) - d_1(0) \| + \Big( \hat{t} + m \frac{ \kappa^{\hat{t} } - \kappa^{t} }{1 - \kappa}\Big) \|  {\bf P} - {\bf P}_1  \|  & t \ge \hat{t}
    \end{cases}
\end{align*}
where $ \hat{t} = \lceil{\log_\kappa m^{-1}}\rceil $. We assume the two state distributions have the same initial state distribution, that is $\rho_0 = d_0$. In addition, 
\begin{equation*}
    \begin{split}
        {\bf P} - {\bf P}_{1} & = q_1{\bf P}_1 + q_2{\bf P}_2 - {\bf P}_{1} \\
        & = (q_1 - 1){\bf P}_1 + (1 - q_1){\bf P}_2 \\
        &= (1 - q_1) ( {\bf P}_2 - {\bf P}_1) 
    \end{split}
\end{equation*}
Then:
\begin{align*}
    \| \rho(t) - d_1(t)\| \le \begin{cases} t (1 - q_1) \|  {\bf P}_2 - {\bf P}_{1}  \| & t < \hat{t} \\ 
    \Big( \hat{t} + m \frac{ \kappa^{\hat{t} } - \kappa^{t} }{1 - \kappa}\Big) \cdot (1 - q_1) \|  {\bf P}_2 - {\bf P}_1  \|  & t \ge \hat{t}
    \end{cases}
\end{align*}

\begin{equation}
    \begin{split}
        \| \rho(t) - \mu_1(\theta)\| & = \| \rho(t) - d_1(t) + d_1(t) - \mu_1(\theta)\| \\
        & \le \| \rho(t) - d_1(t)\| + \| d_1(t) - \mu_1(\theta)\|\\
        & \le \Big( \hat{t} + m \frac{ \kappa^{\hat{t} } - \kappa^{t} }{1 - \kappa}\Big) \cdot (1 - q_1) \|  {\bf P}_2 - {\bf P}_1\| + m\kappa^t
    \end{split}
\end{equation}



\begin{equation}
    \begin{split}
        P = \beta_1 (q_1 P_1^{\theta_1} + q_2 P_2^{\theta_1}) + \beta_2 (q_1 P_1^{\theta_2} + q_2 P_2^{\theta_2})
    \end{split}
\end{equation}
Another try. recall that
\begin{equation*}
    \rho(\tau)^\top = \sum_{k=1}^K \beta_k \sum_{n=1}^N \frac{1}{N} \rho_{t(k,n)}^\top = \sum_{k=1}^K \beta_k \sum_{n-=1}^n \frac{1}{N} \rho_0^\top \prod_{t'=1}^{t(k,n)-1} P_{t'(k',n')}
\end{equation*}
Note that $t(k,n) \in \{0 \ldots \tau-1\}$
\sd{What are t'(k',n') ???}
Note that:
\begin{equation*}
    \rho(\tau+1)^\top = \sum_{k=1}^K \beta_k \sum_{n=1}^N \frac{1}{N} \rho_{t(k,n)}^\top = \sum_{k=1}^K \beta_k \sum_{n-=1}^n \frac{1}{N} \rho_0^\top \prod_{t'=1}^{t(k,n)-1} P_{t'(k',n')} P_{\tau}
\end{equation*}
Then 
\[\rho(t+1)^\top = \rho(t)^\top P_t\]




\sd{A potential problem: $d_1(t)$ has a fixed policy $\pi_\theta$, while in our mixed process we use $\theta_{t(k,n}$ different policies. How do we address that?}

\sd{define which matrix norm}

\end{proof}






==> general.tex <==
\section{XXXX}

\iffalse
We present our algorithm:

\begin{algorithm}
    \caption{Sim2Real-Second}
    \label{alg:s2r_second}
    \begin{algorithmic}[1]
    \ENSURE Two environments $M_{\text{real}}, M_{\text{sim}}$ 
    \STATE Initial actor parameters $\boldsymbol{\theta}_0$, initial critic parameters ${\bf w}_0$, initial average reward estimator $\eta_0$, step size $\alpha^{\theta}_t$ for actor, step size $\alpha^{w}_t$ for critic, and step size $\alpha^{\eta}_t$ for the average reward estimator. 
    \STATE $t=0$ \COMMENT {$t$ is the optimization steps counter}
    \FOR {episode 1, \ldots, $N_{\text{episodes}}$}
        \STATE Sample environment $M_{act}=\{M_{\text{sim}}, M_{\text{real}}\}$ with probability $[p, 1-p]$
        \FOR {step k=1, \ldots, K}
            \STATE Interact with $M_{act}$ according to policy $\pi_b$ and add the transition $\{s_k, a_k, r_k, s_{k+1} \}$ to replay buffer $\mathcal{D}_{M_{act}}$
        \ENDFOR
        \STATE Sample environment for optimization $M_{opt}=\{M_{\text{sim}}, M_{\text{real}}\}$ with probability $[\beta, 1-\beta]$
        \FOR {iteration i=1, \ldots, M}
            \STATE Sample mini-batch $\{s_j, a_j, r_j, s' \}_{j=1}^{N}$ from $\mathcal{D}_{M_{opt}}$
            \STATE $\delta_t = r_t -\eta_t + \phi(s_{t+1})^\top w_t  - \phi(s_{t})^\top w_t   $
            \STATE Update $\eta_{t+1} = \eta_t + \alpha^{\eta}_t (r_t - \eta_t) $
            \STATE Update $w_{t+1} = \Pi_{R_w} \big( w_{t} + \alpha^w_t \delta_t \phi(s_t) \big)  $ \label{line:critic2}
            \STATE Update $\boldsymbol{\theta}_{t+1} = \boldsymbol{\theta}_{t} + \alpha^{\theta}_t \delta_t \nabla_\theta \log \pi_\theta (a_t|s_t)$
            \STATE $t=+1$
        \ENDFOR 
        \STATE Update behaviour policy $\pi_b=\pi_{\theta_t}$
    \ENDFOR 
    \end{algorithmic}
\end{algorithm}

\fi

We present here a linear two-timescale SA (Stochastic approximation)
\begin{equation}
\label{eq:theta}
    \boldsymbol{\theta}_{t+1} = \boldsymbol{\theta}_{t} + \alpha^\theta_t \big(h_1(\boldsymbol{\theta}_{t}, {\bf w}_t) + M_{t+1}^{(1)} \big)
\end{equation}

\begin{equation}
\label{eq:w}
    {\bf w}_{t+1} = {\bf w}_{t} + \alpha^w_t \big(h_2(\boldsymbol{\theta}_{t}, {\bf w}_t) + M_{t+1}^{(2)} \big)
\end{equation}

where $\alpha^\theta_t, \alpha^w_t \in \mathbb{R}$ are step-sizes, $M_{t}^{(i)} \in \mathbb{R}^d$ are noises and $h_i \in \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}^d$ are:
\begin{align*}
    h_i (\boldsymbol{\theta}, {\bf w}) = \nu_i + \Gamma_i \boldsymbol{\theta} + W_i {\bf w}
\end{align*}

where $\nu_i \in \mathbb{R}^d$ and $\Gamma^i, W_i \in \mathbb{R}^{d \times d}$

We assume that:
\begin{assumption}
\label{ass:pd}
$W_2$ and $X_1 = \Gamma_1 - W_1 W_2^{-1} \Gamma_2$ are positive definite (not necessarily symmetric). 
\end{assumption}

\begin{assumption}
The stepsizes sequences $\{\alpha^\theta_t\}$, $\{\alpha^w_t\}$ and $\{\eta_t := \alpha^\theta_t / \alpha^w_t \}$ satisfy:
\[\sum_{t=0}^{\infty} \alpha^\theta_t =  \sum_{t=0}^{\infty} \alpha^w_t = \infty\]

\[\alpha^\theta_t, \alpha^w_t, \eta_t \le 1\]
and
\[\lim_{t \rightarrow \infty} \alpha^\theta_t = \lim_{t \rightarrow \infty} \alpha^w_t = \lim_{t \rightarrow \infty} \eta_t = 0 \]
\end{assumption}

\begin{assumption}
$\{ M_{t}^{(1)} \}$ and $\{ M_{t}^{(2)} \}$ are martingale difference sequences w.r.t the family of $\sigma$-fields $\{\mathcal{F}_t\}$ where $\mathcal{F}_t = \sigma \big( \boldsymbol{\theta}_0, {\bf w}_0, M_{1}^{(1)}, M_{1}^{(2)}, \ldots, M_{t}^{(1)}, M_{t}^{(2)} \big)$. There exist constants $m_1, m_2 > 0$ so that $\| M_{t+1}^{(1)}\| \le m_1 (1 + \| \boldsymbol{\theta}_t\| + \| {\bf w}_t\|) $ and $\| M_{t+1}^{(2)}\| \le m_2 (1 + \| \boldsymbol{\theta}_t\| + \| {\bf w}_t\|) $ for all $t \ge 0$.
\end{assumption}

We outline the ODE method from (Borkar, 2008, pp. 64-65) for the analysis of Equations (\ref{eq:theta}) and (\ref{eq:w}). Since $\eta_t \rightarrow 0$,  $\{{\bf w}_t\}$ is the fast transient
and $\{ \boldsymbol{\theta}_t\}$ is the slow component. Therefore, the ODE that (\ref{eq:w}) might be expected to track is:
\begin{equation}
\label{eq:w_dot}
    {\bf \dot{w}}(t) = \nu_2 - \Gamma_2 \boldsymbol{\theta} - W_2 {\bf w}(t)
\end{equation}

for some foxed $\boldsymbol{\theta}$ and the ODE that (\ref{eq:theta}) might be expected to track is:
\begin{equation}
\label{eq:theta_dot}
    \dot{\boldsymbol{\theta}} (t) = h_1 \big( \boldsymbol{\theta}_t, \lambda(\boldsymbol{\theta}_t) \big) = {\bf b}_1 - X_1 \boldsymbol{\theta}(t)
\end{equation}
\[\]
where ${\bf b}_1 = \nu_1 - W_1 W_2^{-1} \nu_2$ and $\lambda(\boldsymbol{\theta}) = W_2^{-1} (\nu_2 - \gamma_2 \boldsymbol{\theta})$. Due to Assumption \ref{ass:pd}, $\lambda(\boldsymbol{\theta})$ and ${\bf b}_1$ are well defined.  Moreover, $\lambda(\boldsymbol{\theta})$  and $\boldsymbol{\theta}^* := X_1^{-1} {\bf b}_1$ are unique globally asymptotically stable equilibrium points of (\ref{eq:w_dot}) and (\ref{eq:theta_dot}), respectively.

\subsection{SA for sim2real}
Consider the following:
Let
\[C_t^{\text{sim}} = \phi (s_t^{\text{sim}}) \big(\gamma \phi(s_{t+1}^{\text{sim}}) - \phi(s_t^{\text{sim}})\big)^\top\]
\[C_t^{\text{real}} = \phi (s_t^{\text{real}}) \big(\gamma \phi(s_{t+1}^{\text{real}}) - \phi(s_t^{\text{real}})\big)^\top\]
\[d_t^{\text{sim}} = r_t^{\text{sim}} \phi(s_t^{\text{sim}})\]
\[d_t^{\text{real}} = r_t^{\text{real}} \phi(s_t^{\text{real}})\]
\[ \boldsymbol{\theta}_{t+1} = \boldsymbol{\theta}_t - \alpha^\theta_t \Big( \beta \cdot  C_t^{\top \text{sim}} + (1 - \beta)C_t^{\top \text{real}} \Big) {\bf w}_t\]
\[{\bf w}_{t+1} = {\bf w}_t + \alpha^w_t \Big( \beta \cdot  d_t^{\text{sim}} + (1 - \beta)d_t^{\text{real}} + \big( \beta \cdot  C_t^{\text{sim}} + (1 - \beta)C_t^{\text{real}} \big) \boldsymbol{\theta}_t\Big)\]

In this case we have:
\[ h_1 (\boldsymbol{\theta}, {\bf w}) = {\bf A}^\top {\bf w}\]
\[\nu_1 = {\bf 0}\]
\[\Gamma_1 = {\bf 0}\]
\[W_1 = - {\bf A}^T\]

\[ h_2 (\boldsymbol{\theta}, {\bf w}) = {\bf b} - {\bf A}\boldsymbol{\theta} - {\bf w}\]
\[\nu_2 = {\bf b}\]
\[\Gamma_2 = {\bf A}\]
\[W_2 = {\bf I}\]

where 
\begin{align*}
    {\bf A} & = \beta \mathbb{E}_{s, s' \sim M_{\text{sim}}} \big[\phi (s^{\text{sim}}) \big(\gamma \phi(s'^{\text{sim}}) - \phi(s^{\text{sim}})\big)^\top \big] \\
    & + (1 - \beta) \mathbb{E}_{s, s' \sim M_{\text{real}}} \big[\phi (s^{\text{real}}) \big(\gamma \phi(s'^{\text{real}}) - \phi(s^{\text{real}})\big)^\top \big]
\end{align*}





\[ {\bf b} =  \beta \mathbb{E}_{s, r \sim M_{\text{sim}}} \big[r^{\text{sim}} \phi (s^{\text{sim}})  \big] + (1 - \beta) \mathbb{E}_{s, r \sim M_{\text{real}}} \big[r^{\text{real}} \phi (s^{\text{real}})  \big] \]

Let's define:
\[{\bf A}_{\text{sim}} = \mathbb{E}_{s, s' \sim M_{\text{sim}}} \big[\phi (s^{\text{sim}}) \big(\gamma \phi(s'^{\text{sim}}) - \phi(s^{\text{sim}})\big)^\top \big]\]

\[{\bf A}_{\text{real}} = \mathbb{E}_{s, s' \sim M_{\text{real}}} \big[\phi (s^{\text{real}}) \big(\gamma \phi(s'^{\text{real}}) - \phi(s^{\text{real}})\big)^\top \big]\]

\[ {\bf b}_{\text{sim}} =  \mathbb{E}_{s, r \sim M_{\text{sim}}} \big[r^{\text{sim}} \phi (s^{\text{sim}})  \big] \]

\[ {\bf b}_{\text{real}} =  \mathbb{E}_{s, r \sim M_{\text{real}}} \big[r^{\text{real}} \phi (s^{\text{real}})  \big] \]

Then, we can write:
\[ {\bf A} = \beta {\bf A}_{\text{sim}} + (1-\beta) {\bf A}_{\text{real}}\]
\[ {\bf b} = \beta {\bf b}_{\text{sim}} + (1-\beta) {\bf b}_{\text{real}}\]

Let's look at:
\begin{align*}
    X_1 & = \Gamma_1 - W_1 W_2^{-1} \Gamma_2\\
    & = {\bf A}^T {\bf A} \\
    & = \big(  \beta {\bf A}_{\text{sim}} + (1-\beta) {\bf A}_{\text{real}} \big)^\top \big(  \beta {\bf A}_{\text{sim}} + (1-\beta) {\bf A}_{\text{real}} \big) \\
    & = \beta^2 {\bf A}_{\text{sim}}^\top {\bf A}_{\text{sim}} + (1-\beta)^2 {\bf A}_{\text{real}}^\top {\bf A}_{\text{real}} \\
    & + \beta (1-\beta) \big( {\bf A}_{\text{sim}}^\top {\bf A}_{\text{real}} + {\bf A}_{\text{real}}^\top {\bf A}_{\text{sim}} \big)
\end{align*}
We Assume $X_1$ is positive definite (PD). Note that sum of PD and PD is PD, and that transpose of PD is PD. 

 \newpage
\subsection{Asymptotic Convergance}
**** PRESENT AUXILLARY MDP and show that it is equivilent to :

Let $M^\beta_{\text{s2r}}$ be an MDP with transition probability that takes the form:
\[P^\beta_{\text{s2r}} (s'|s, a) = \beta P_\text{sim}(s'|s, a) + (1 - \beta) P_{\text{real}}(s'|s, a)\]
$P^\beta_{\text{s2r}}(s'|s)$ is the associate Markov chain of MDP $M_{\text{s2r}}$ and it is ergodic:
\[P^\beta_{\text{s2r}}(s'|s) = \sum_{a \in \mathcal{A}} P^\beta_{\text{s2r}} (s'|s, a) \pi(a|s)\]

$\mu_{\text{s2r}(\beta)}^\pi$ is the stationary distribution, induced by policy $\pi$, which satisfies the following recursion:

\[\mu_{\text{s2r}(\beta)}^\pi (s') = \sum_{s \in \mathcal{S}} P^\beta_{\text{s2r}}(s'|s) \mu_{\text{s2r} (\beta)}^\pi (s) \]


In this work we consider the “average reward” setting (Sutton et al., 2000), where under the ergodicity assumption, the average reward over time eventually converges to the expected reward under the stationary distribution:

\[r_{\text{s2r}}(\boldsymbol{\theta}) := \lim_{N \rightarrow \infty} \frac{\sum_{t=0}^N r(s_t, a_t)}{N} = \mathbb{E}_{s \sim \mu_{\text{s2r}(\beta)}^{\pi_\theta}, a \sim \pi_{\theta}} [r(s,a)]\]

We will follow notations from \cite{wu2020finite}. However, note that our $r_{\text{s2r}}(\boldsymbol{\theta})$ is based on the MDP $M^\beta_{\text{s2r}}$ that combines samples from both sim and real environments. 

To evaluate the overall rewards given a starting state $s$ and the behavior policy $\pi_\theta$, we define the state-value function as

XXXXXXXXX We need to deciede if this definition: XXXXXXXX
\begin{align*}
    V^{\pi_\theta} (s) & :=  \mathbb{E}^\beta_{\text{s2r}} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, \pi_\theta \big] \\
    & = \beta \mathbb{E}_{\text{sim}} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big)| s_0=s, \pi_\theta \big] \\
    & + (1-\beta) \mathbb{E}_{\text{real}} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t)  - r_{\text{s2r}}(\boldsymbol{\theta}) \big)| s_0=s, \pi_\theta \big] 
\end{align*}

where the action follows the policy $a_t \sim \pi_\theta(\cdot|s_t)$ and the next state follows the transition probability $s_{t+1} \sim P^\beta_{\text{s2r}}(\cdot|s_t, a_t)$. Another frequently used function is the state-action value function, also called Q-value function:

\begin{align*}
    & Q^{\pi_\theta} (s,a) :=  \mathbb{E}^\beta_{\text{s2r}} \big[ \sum_{t=0}^{\infty} \big(r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, a_0=a, \pi_\theta \big] \\
    & = \beta \mathbb{E}_{\text{sim}} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, a_0=a, \pi_\theta \big] \\
    & + (1-\beta) \mathbb{E}_{\text{real}} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, a_0=a, \pi_\theta \big] \\
    & = \beta r_\text{sim}(s,a) + (1-\beta) r_{\text{real}}(s,a) - r_{\text{s2r}}(\boldsymbol{\theta}) + \mathbb{E}^\beta_{\text{s2r}} \big[ V^{\pi_\theta} (s') \big]
\end{align*}

where the expectation $\mathbb{E}^\beta_{\text{s2r}}$ is taken over $s' \sim P^\beta_{\text{s2r}}(\cdot|s, a)$.

XXXXXXXX Or this definition: XXXXXXXXXXXX

\begin{align*}
    V^{\pi_\theta}_{\text{real}} (s) & :=  \mathbb{E} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, \pi_\theta \big] \\
\end{align*}

\begin{align*}
    V^{\pi_\theta}_{\text{sim}} (s) & :=  \mathbb{E} \big[ \sum_{t=0}^{\infty} \big( r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, \pi_\theta \big] \\
\end{align*}

where the action follows the policy $a_t \sim \pi_\theta(\cdot|s_t)$ and the next state follows the transition probability $s_{t+1} \sim P_{\text{real}}(\cdot|s_t, a_t)$ or $s_{t+1} \sim P_{\text{real}}(\cdot|s_t, a_t)$ respectively. Another frequently used function is the state-action value function, also called Q-value function:

\begin{align*}
    Q^{\pi_\theta}_{\text{real}} (s,a) & :=  \mathbb{E} \big[ \sum_{t=0}^{\infty} \big(r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, a_0=a, \pi_\theta \big] \\
    & = r_\text{real}(s,a) - r_{\text{s2r}}(\boldsymbol{\theta}) + \mathbb{E} \big[ V^{\pi_\theta}_{\text{real}} (s') \big]
\end{align*}

\begin{align*}
    Q^{\pi_\theta}_{\text{sim}} (s,a) & :=  \mathbb{E} \big[ \sum_{t=0}^{\infty} \big(r(s_t, a_t) - r_{\text{s2r}}(\boldsymbol{\theta}) \big) | s_0=s, a_0=a, \pi_\theta \big] \\
    & = r_\text{sim}(s,a) - r_{\text{s2r}}(\boldsymbol{\theta}) + \mathbb{E} \big[ V^{\pi_\theta}_{\text{sim}} (s') \big]
\end{align*}

where the expectation $\mathbb{E}$ is taken over $s' \sim P_{\text{real}}(\cdot|s, a)$ or $s' \sim P_{\text{sim}}(\cdot|s, a)$ respectively.

XXXXXXX Continue

We define the performance function associated with policy $\pi_\theta$ naturally as the expected reward under the stationary distribution $\mu_{\text{s2r}(\beta)}^{\pi_\theta}$ induced by $\pi_\theta$, which takes the form
\begin{equation}
\label{objective}
    J(\theta) := r_{\text{s2r}}(\theta)
\end{equation}
To maximize the performance function with respect to the policy parameters, Sutton et al. (2000) proved the following policy gradient theorem ..... 

The gradient of $J(\theta)$ takes the form:

XXXXX We need to decide if this: XXXXXX
\begin{align*}
    \nabla J(\boldsymbol{\theta}) & = \mathbb{E}_{s \sim \mu_{\text{s2r}(\beta)}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta} (s,a) \nabla \log \pi_\theta (a|s) \big] \\
    & = \beta \mathbb{E}_{s \sim \mu_{\text{sim}}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta} (s,a) \nabla \log \pi_\theta (a|s) \big] \\
    & + (1 - \beta) \mathbb{E}_{s \sim \mu_{\text{real}}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta} (s,a) \nabla \log \pi_\theta (a|s) \big]
\end{align*}

XXXXX Or this: XXXXXX
\begin{align*}
    \nabla J(\boldsymbol{\theta}) & = \mathbb{E}_{s \sim \mu_{\text{s2r}(\beta)}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta} (s,a) \nabla \log \pi_\theta (a|s) \big] \\
    & = \beta \mathbb{E}_{s \sim \mu_{\text{sim}}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta}_{\text{sim}} (s,a) \nabla \log \pi_\theta (a|s) \big] \\
    & + (1 - \beta) \mathbb{E}_{s \sim \mu_{\text{real}}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta}_{\text{real}} (s,a) \nabla \log \pi_\theta (a|s) \big]
\end{align*}
 XXXXX Both are not true!!! since we cannot decompose $\mu_{\text{s2r}(\beta)}^{\pi_\theta}$ into $\beta \mu_{\text{sim}}^{\pi_\theta} + (1-\beta) \mu_{\text{real}}^{\pi_\theta} $ XXXXX
 
Now consider the case in which the action-value function for a fixed policy $\pi_\theta$, $Q^{\pi_\theta}$, is approximated by a learned function approximator. Sutton et al. (citeXXX) showed that if the approximation $\hat{Q}^{\pi_\theta}_{{\bf w}}$ with parameter ${\bf w} \in \mathbb{R}^d$ is compatible, i.e., $\nabla_w Q^{\pi_\theta}_{w}(s,a) = \nabla \log \pi_\theta(a|s)$, and minimizes the mean squared error:
\[\mathcal{E}^{\pi_\theta} ({\bf w}) = \mathbb{E}_{s \sim \mu_{\text{s2r}(\beta)}^{\pi_\theta}, a \sim \pi_{\theta}} \big[ (Q^{\pi_\theta} - \hat{Q}^{\pi_\theta}_{{\bf w}})^2 \big]\]

for parameter value ${\bf w}^*$, then we can replace $Q^{\pi_\theta}$ with $\hat{Q}^{\pi_\theta}_{{\bf w}^*}$. We work with linear approximation $\hat{Q}^{\pi_\theta}_{{\bf w}} = {\bf w}^\top \phi(s,a)$ in which the $\phi(s,a)$’s are compatible features defined according to $\phi(s,a) = \nabla \log \pi (a|s)$.

XXXXXXXXXXXXXXXX


Consider the following function $f^\text{s2r}$ parameterized by $\theta \in \mathbb{R}^d$, $\forall s, a$:
\[f_\theta^\text{s2r} (s,a) = \begin{cases} r_\text{real} (s,a) + \gamma V_\theta'(s'_\text{real}) - V_\theta(s) & \text{w.p. } (1 - \beta) \\
                                    r_\text{sim} (s,a) + \gamma V_\theta'(s'_\text{sim}) - V_\theta(s) & \text{w.p. } \beta \end{cases} \]
The gradient $\nabla^\theta f_\theta^\text{s2r} (s,a)$ is then:
\[ \nabla^\theta f_\theta^\text{s2r} (s,a) = - \nabla^\theta  V_\theta(s)\]
Consider the error for $(s,a)$:
\[g_\theta^\text{s2r} (s,a) = \frac{1}{2} \big( f_\theta^\text{s2r} (s,a) \big)^2 \]
and its gradient:
\[\nabla^\theta g_\theta^\text{s2r} (s,a) =  f_\theta^\text{s2r} (s,a) \cdot \nabla^\theta f_\theta^\text{s2r} (s,a)\]
and consider the expectation over this error, meaning the mean square error loss function $\bar{g}_\theta^\text{s2r}$:
\[\bar{g}_\theta^\text{s2r} = \mathbb{E}_{s,a \sim M_\text{real} \cup M_\text{sim}}[g_\theta^\text{s2r}(s,a)] = \mathbb{E}_{s,a \sim M_\text{real} \cup M_\text{sim}} \big[ \frac{1}{2} \big( f_\theta^\text{s2r} (s,a) \big)^2 \big]\]
Note that the $\sigma-\text{algebra}$ is the cross product of $M_{\text{real}} \times M_{\text{sim}}$. However, the actual samples will come from a smaller subset, which contains only samples from pure $M_{\text{real}}$ and pure $M_{\text{sim}}$. 
By the law of total expectation:
\begin{align*}
    \bar{g}_\theta^\text{s2r} & = \mathbb{E} \big[ \frac{1}{2} \big( f_\theta^\text{s2r} (s,a) \big)^2 \big] = \sum_{M=M_\text{real}, M_\text{sim}} P(M) \mathbb{E} \big[ \frac{1}{2} \big( f_\theta^\text{s2r} (s,a) \big)^2 | M\big] \\
                        & = (1 - \beta) \cdot \mathbb{E}_{M_\text{real}} \big[ \frac{1}{2} \big( r_\text{real} (s,a) + \gamma V_\theta'(s'_\text{real}) - V_\theta(s) \big)^2 \big]\\
                        & + \beta \cdot \mathbb{E}_{M_\text{sim}} \big[ \frac{1}{2} \big( r_\text{sim} (s,a) + \gamma V_\theta'(s'_\text{sim}) - V_\theta(s) \big)^2 \big]
\end{align*}
The gradient $\nabla^\theta \bar{g}_\theta^\text{s2r}$ is then:
\begin{align*}
    \nabla^\theta \bar{g}_\theta^\text{s2r}   & = \mathbb{E} [\nabla^\theta g_\theta^\text{s2r} (s,a)]\\
                                        & = \mathbb{E} \big[ f_\theta^\text{s2r} (s,a) \cdot \nabla^\theta f_\theta^\text{s2r} (s,a) \big]\\
                                        & = (1 - \beta) \cdot \mathbb{E}_{M_\text{real}} \big[ - \nabla^\theta  V_\theta(s) \big( r_\text{real} (s,a) + \gamma V_\theta'(s'_\text{real}) - V_\theta(s) \big) \big]\\
                                        & + \beta \cdot \mathbb{E}_{M_\text{sim}} \big[ - \nabla^\theta  V_\theta(s) \big( r_\text{sim} (s,a) + \gamma V_\theta'(s'_\text{sim}) - V_\theta(s) \big) \big]
\end{align*}

We now consider a stochastic approximation update for $\theta$. We seek to minimize the mean square error $\bar{g}_\theta^\text{s2r}$ by gradient descent, given by: 
\begin{align*}
    \theta_{t+1} & = \theta_t -\nabla^\theta \bar{g}_{\theta_t}^\text{s2r}
\end{align*}
Since the expectation cannot be evaluated, we may approximate it with the 'empirical gradient' at $(s_t, a_t)$:
\begin{align*}
    \theta_{t+1} & = \theta_t - \nabla^\theta g_{\theta_t}^\text{s2r} (s_t, a_t)\\
                & = \theta_t - f_{\theta_t}^\text{s2r} (s_t,a_t) \cdot \nabla^\theta f_{\theta_t}^\text{s2r} (s_t,a_t) 
\end{align*}

Since this scheme is a correlated random walk, we would like to smooth it by making only a small, incremental move in the direction suggested by the gradient instead of making the full move (making a convex combination of previous estimation and new gradient step):
\begin{align}
\label{gradient_step}
    \theta_{t+1} & = (1 - \alpha_t) \theta_t + \alpha_t \big( - \nabla^\theta g_{\theta_t}^\text{s2r} (s_t, a_t) \big) 
\end{align}
 Now let’s add and subtract the exact error gradient $\nabla^\theta \bar{g}_{\theta_t}^\text{s2r} = \mathbb{E}_{s,a \sim M_\text{real} \cup M_\text{sim}}[\nabla^\theta g_\theta^\text{s2r}(s,a)]$ at the ‘known guess’ $\theta_t$ from the empirical gradient on the right-hand side and rewrite the above scheme as :
 \begin{align*}
     \theta_{t+1} & = (1 - \alpha_t) \theta_t + \alpha_t \big( - \mathbb{E}[\nabla^\theta g_{\theta_t}^\text{s2r}(s,a)] - \nabla^\theta g_{\theta_t}^\text{s2r} (s_t, a_t) + \mathbb{E}[\nabla^\theta g_{\theta_t}^\text{s2r}(s,a)] \big) 
 \end{align*}
This is of the form
\begin{align*}
     \theta_{t+1} & = (1 - \alpha_t) \theta_t + \alpha_t \big( h_\theta + M_{t+1} \big) 
 \end{align*}
where 
\[h_\theta = - \mathbb{E}[\nabla^\theta g_{\theta_t}^\text{s2r}(s,a)] = - \nabla^\theta \bar{g}_{\theta_t}^\text{s2r}\] 
\[M_{t+1} = \mathbb{E}[\nabla^\theta g_{\theta_t}^\text{s2r}(s,a)] - \nabla^\theta g_{\theta_t}^\text{s2r} (s_t, a_t)\]
with $\{ M_t\}$ a martingale diﬀerence sequence.



\begin{theorem}

\end{theorem}
\section{Notes}
The product of two symmetric PSD matrices is PSD, iff the product is also symmetric. More generally, if A and B are PSD, AB is PSD iff AB is normal, ie. $(AB)^T AB = AB (AB)^T$. 

Reference: On a product of positive semidefinite matrices, A.R. Meenakshi, C. Rajian, Linear Algebra and its Applications, Volume 295, Issues 1–3, 1 July 1999, Pages 3–6.

\newpage
\section{Stationary distribution}
Let: $\mu_1$, $\mu_2$ be stationary distributions satisfying:
\[\mu_1 = \mu_1 P_1\]
\[\mu_2 = \mu_2 P_2\]

Let $\mu$ be a convex combination of these disributions ($\beta \in [0,1]$)
\begin{align*}
    \mu & = \beta \mu_1 + (1-\beta) \mu_2 \\
    & = \beta \mu_1 P_1 + (1-\beta) \mu_2 P_2 \\
    & = \mu_2 P_2 + \beta (\mu_1 P_1 - \mu_2 P_2) + (1 - \beta) \mu_2 P_1 - (1 - \beta) \mu_2 P_1 \\
    & = \mu_2 P_2  -\mu_2 \big( \beta P_2 + (1-\beta) P_1 \big) + \big( \beta \mu_1 + (1-\beta) \mu_2 \big) P_1 \\
    & = \mu_2 P_2  -\mu_2 \big( \beta P_2 + (1-\beta) P_1 \big) + \mu P_1
\end{align*}

Then:
\[\boxed{\mu = \beta \mu_1 + (1-\beta) \mu_2 = \mu_2 P_2  -\mu_2 \big( \beta P_2 + (1-\beta) P_1 \big) + \mu P_1}\]

If we further continue:

\begin{align*}
    \mu & = \mu_2 P_2  -\mu_2 \big( \beta P_2 + (1-\beta) P_1 \big) + \mu P_1\\
    \mu (I - P_1) & = \mu_2 \big( (1 - \beta) P_2 - (1-\beta) P_1 \big) \\
    \mu (I - P_1) & = (1 - \beta) \mu_2 \big(  P_2 -  P_1 \big)\\
    \mu  & = (1 - \beta) \mu_2 \big(  P_2 -  P_1 \big) (I - P_1)^{-1}
\end{align*}

Then:
\[\boxed{\mu  = (1 - \beta) \mu_2 \big(  P_2 -  P_1 \big) (I - P_1)^{-1}}\]



==> lemma1_dotan_version.tex <==
\subsection{Proof of Lemma \ref{lemma:RB_is_markovian}}
%\newcommand{\OO}{\tilde{\mathcal{O}}}
\begin{proof}
\textbf{1.} Proving Markovity requires that
\begin{equation}
\label{eq:X_definition_of_markov}
    P(X_{\tau+1}|X_{\tau}, X_{\tau-1}, \ldots, X_0) = P(X_{\tau+1}|X_{\tau}).
\end{equation}
Let us denote $\OO_{n_1}^{n_2} \triangleq \{\OO_{n_1}, \ldots, \OO_{n_2}\}$ and $s_{n_1}^{n_2} \triangleq \{s_{n_1}, \ldots, s_{n_2}\}$. Computing the l.h.s. of \eqref{eq:X_definition_of_markov} yields
\begin{equation*}
    \begin{split}
        P(X_{\tau+1}|X_{\tau}, X_{\tau-1}, \ldots, X_0) 
        &\stackrel{1}{=} 
        P(s_{\tau+1}, RB_{\tau+1}| s_{\tau}, RB_{\tau}, \ldots, s_{0}, RB_{0})\\
        &\stackrel{2}{=}  
        P(s_{\tau+1}, \OO_{\tau-N+1}^{\tau}| s_{\tau}, \OO_{\tau-N}^{\tau-1}, \ldots, s_{0}, \OO_0)\\
        &\stackrel{3}{=} 
        P(s_{\tau+1}, \OO_{\tau-N+1}^{\tau}| s_{0}^{\tau}, \OO_{0}^{\tau-1})\\   
        &\stackrel{4}{=} 
        P(s_{\tau+1}| s_{0}^{\tau+1}) \times P(\OO_{\tau-N+1}^{\tau}| s_{0}^{\tau}, \OO_{0}^{\tau-1}) \\
        &\stackrel{5}{=} 
        P(\OO_{\tau}, \OO_{\tau-N+1}^{\tau-1}| \OO_{0}^{\tau-1}) \\
        &=
        P(\OO_{\tau}| \OO_{\tau-N}^{\tau-1}). \\
    \end{split}
\end{equation*}        
where in equality (1) we use the definition, in equality (2) we wrote the RB samples explicitly, in equality (3) the terms were rearrange, in equality (4) we expressed the probability as a product, and in equality (5) $s_{\tau+1}$ is conditioned on $s_{\tau+1}$ and we use the fact that $s_0^{\tau} \subset \OO_{0}^{\tau-1}$. Similarly, computing the r.h.s of \eqref{eq:X_definition_of_markov} yields
\begin{equation*}
    \begin{split}
        P(X_{\tau+1}|X_{\tau}) 
        &= 
        P(s_{\tau+1}, RB_{\tau+1}| s_{\tau}, RB_{\tau})\\
        &= 
        P(s_{\tau+1}| s_{\tau+1}, RB_{\tau}) \times P(RB_{\tau+1}| s_{\tau}, RB_{\tau})\\
        &= 
        P(\OO_{\tau}| \OO_{\tau-N}^{\tau-1}).\\
    \end{split}
\end{equation*}
Both sides of \eqref{eq:X_definition_of_markov} are equal and therefore $X_\tau$ is Markovian.

\textbf{2.} We assume that for every policy $\pi$ the induced Markov Reward Process induced by the MDP together with the policy $\pi$ is irreducible and aperiodic. We show that the induced transition $P(X_{\tau+1}|X_{\tau})$ has the same probability measure as $P(s_{\tau+1}|s_\tau)$. In part \textbf{1} the transition of the RB is provided explicitly. Rearranging terms yields
\begin{equation*}
    \begin{split}
        P(\OO_{\tau}| \OO_{\tau-N}^{\tau-1})
        &=
        P(s_\tau, a_\tau, r_\tau, s_{\tau+1} | s_{\tau-N}^{\tau}, a_{\tau-N}^{\tau-1},r_{\tau-N}^{\tau-1}) \\
        &=
        P(a_\tau, r_\tau, s_{\tau+1} | s_{\tau-N}^{\tau}, a_{\tau-N}^{\tau-1},r_{\tau-N}^{\tau-1}) \times P(s_{\tau} | s_{\tau-N}^{\tau}, a_{\tau-N}^{\tau-1},r_{\tau-N}^{\tau-1}) \\
        &=
        P(a_\tau, r_\tau, s_{\tau+1} | s_{\tau}) \\
        &=
        P(r_\tau, s_{\tau+1} | s_{\tau}, a_\tau) \times  P(a_\tau| s_{\tau})\\    
        &=
        P(s_{\tau+1} | s_{\tau}, a_\tau) \times P(r_{\tau} | s_{\tau}, a_\tau) \times \pi_\theta(a_\tau| s_{\tau}).\\
    \end{split}
\end{equation*}
Since the probability $P(r_{\tau} | s_{\tau}, a_\tau)$
\end{proof}

==> nomenclature.tex <==
\onecolumn
\section{Nomenclature}
\begin{table}[ht]
\centering
\resizebox{1.00\linewidth}{!}{%
\begin{tabular}{l|l}
Symbol & description \\
\hline \hline \\
$t$ & The time the observation occured \\
$\tau$ & The time of sampling an observation \\
$K$ & Number of MDPs the agent interact with \\
$\beta_i$ & probability of choosing $\text{RB}(i)$ \\
$q_i$ & probability of sampling from / interacting with MDP $i$ \\
$RB; RB(i); RB_\tau; RB_\tau(i)$ & Replay buffer; Replay buffer storing samples from\\
& MDP i; The content of the replay buffer at time $\tau$.\\
$P(\cdot|\cdot, \cdot); P_i(\cdot|\cdot, \cdot)$ & Transition probability of MDP M; of MDP $M_i$.\\
$\alpha_\tau^\eta; \alpha_\tau^v, \alpha_\tau^\theta$ & learning rates for updating parameters $\eta, v, \theta$. \\
$\mathcal{O}_{\tau} = \{s_{\tau}, a_{\tau}, s_{\tau+1}, r_{\tau}\}$ & A transition in the Markov chain.\\
$\tilde{\mathcal{O}}_{\tau,t,i} = \{\tilde s_{\tau, t}, \tilde a_{\tau, t}, \tilde s_{\tau,t+1}, \tilde r_{\tau,t}\}$ & A transition sampled at time $\tau$ from $RB(i)$.\\
& The index $t$ refers to the time-setp when the sample\\
& entered $RB(i)$.\\
$I; I_\tau$ & A Bernoulli random variable that selects which $RB$ \\
& to sample from; The value sampled at time $\tau$. 
\end{tabular}
}
\caption{Nomenclature for the paper}
\label{tab:CVRP-results}
\end{table}


==> obselete.tex <==
\section{Appendix}
\subsection{critic analysis}
We begin with the following assumption (XXX Place it earlier in the paper):
\begin{assumption}
\label{ass:ergodic}
Under any policy $\pi$, the Markov chain resulting from the MDP, $\{s_t, t= 0, 1, 2, \ldots \}$ is irreducible and aperiodic.
\end{assumption}



Let $\mu^{\pi_\theta}_{i}$ be the stationary distribution for MDP $M_i$, induced by the policy $\pi_\theta$. Let $Q^{\pi_\theta}_{i}$ be the Q-function of MDP $M_i$. We use the same parameter ${\bf w}$ for all  $Q^{\pi_\theta}_{i}$'s. Let $J_i(\boldsymbol{\theta}$ be the average reward for MDP $M_i$. In our setup, the loss for the critic is a convex combination of the losses of each one of the agents $A_i$:  

\begin{align*}
    \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) & = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \frac{1}{2} \big( Q^{\pi_\theta}_i(s,a) - \hat{Q}^{\pi_\theta}_{i,{\bf w}} (s,a) \big)^2 \big] \\
\end{align*}
The gradient is then
\begin{align*}
    \nabla_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) & = - \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \big( Q^{\pi_\theta}_i (s,a) - \hat{Q}^{\pi_\theta}_{i, {\bf w}}(s,a) \big) \nabla_{{\bf w}} \hat{Q}^{\pi_\theta}_{i, {\bf w}}(s,a) \big] \\
\end{align*}
We estimate this gradient by a single transition sample from each one of the MDPs $\{s_i, a_i, s_i'\}_{i=1}^K$
\begin{align*}
    \hat \nabla_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) & =  - \sum_{i=1}^K \beta_i \big( Q^{\pi_\theta}_i (s_i,a_i) - \hat{Q}^{\pi_\theta}_{i, {\bf w}}(s_i,a_i) \big) \nabla_{{\bf w}} \hat{Q}^{\pi_\theta}_{i, {\bf w}}(s_i,a_i) \\
\end{align*}

Similarly:
\[J_{\text{s2r}}(\boldsymbol{\theta}) = r _{\text{s2r}}(\boldsymbol{\theta}) = \sum_{i=1}^K \beta_i J_i(\boldsymbol{\theta}) =  \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} [r(s,a)]\]

The gradient is then: 
\[\nabla J_{\text{s2r}}(\boldsymbol{\theta}) = \sum_{i=1}^K \beta_i \nabla J_i(\boldsymbol{\theta}) \]
where
\[\nabla J_i(\boldsymbol{\theta}) = \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} [\nabla \log \pi (a|s) Q^{\pi_\theta}_i (s,a)] \]
Observe that if $b_i(s)$ are any given function of s (also called a baselines), then
\begin{align*}
    & \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} [\nabla \log \pi (a|s) b_i (s)]\\
    & = \sum_{i=1}^K \beta_i \Big( \sum_s \mu^{\pi_\theta}_{i}(s) b_i (s) \nabla \big( \sum_a \pi (a|s) \big)  \Big) \\
      & = \sum_{i=1}^K \beta_i \Big( \sum_s \mu^{\pi_\theta}_{i}(s) b_i (s) \nabla \big( 1 \big)  \Big) = 0
\end{align*}
and thus, for any baselines $b_i(s)$, the gradient of the average reward can be written as
\[\nabla J_{\text{s2r}}(\boldsymbol{\theta}) = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[\nabla \log \pi (a|s) \big( Q^{\pi_\theta}_i (s,a) \pm  b_i(s) \big) \big] \]

The baselines $b_i(s)$ can be chosen in a way that the variance of the gradient estimates $\nabla J_{\text{s2r}}(\boldsymbol{\theta})$ is minimized (cite XXXX).

The Fisher information matrix of Equation XXX can be written using the compatible features as
\begin{align*}
    G_{\text{s2r}} (\boldsymbol{\theta}) & = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \nabla \log \pi (a|s) \nabla \log \pi (a|s)^\top \big] \\
    & = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \psi(s,a) \psi(s,a)^\top \big] 
\end{align*}


Suppose $\mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w})$ denotes the mean squared error:
\begin{align*}
    \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) & = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \frac{1}{2} \big( Q^{\pi_\theta}_i(s,a) - {\bf w}^\top \psi(s,a) - b_i(s) \big)^2 \big] \\
\end{align*}
of our compatible linear parameterized approximation ${\bf w}^\top \psi(s,a)$ and arbitrary baselines $b_i(s)$. Let ${\bf w}^* = \arg \min_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w})$ denote the optimal parameter. We first show in Lemma XXXX that the value
of ${\bf w}^*$ does not depend on the given baselines $b_i(s)$; as a result the mean squared error problems of Equations XXX and XXX have the same solutions. 

\begin{lemma}
The optimum weight parameter ${\bf w}^*$ for any given $\boldsymbol{\theta}$ (policy $\pi$) satisfies:
\[{\bf w}^* = G_{\text{s2r}} (\boldsymbol{\theta})^{-1} \Big( \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ Q^{\pi_\theta}_i(s,a) \psi(s,a) )\big] \Big) \]
\end{lemma}

\begin{proof}
Note that:
\begin{align*}
    \nabla_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) & = - \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \big( Q^{\pi_\theta}_i (s,a) \\
    & - {\bf w}^\top \psi(s,a) - b_i(s) \big) \psi(s,a) \big]
\end{align*}

For the optimal parameter ${\bf w}^*$ we have $\nabla_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}^*) = 0$. Then:
\begin{align*}
    & \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[ \psi(s,a) \psi(s,a)^\top {\bf w}^* \big] \\
    & = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[  Q^{\pi_\theta}_i (s,a) \psi(s,a) \big]\\
    & - \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[  b_i (s) \psi(s,a) \big] 
\end{align*}
Recall that the features are compatible, meaning $\psi(s,a) = \nabla \log \pi (a|s)$. The last term on the right hand side equals zero because:
\begin{align*}
    & \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[  b_i (s) \psi(s,a) \big] \\
     & \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi_\theta}_{i}, a \sim \pi_{\theta}} \big[  b_i (s) \nabla \log \pi (a|s) \big] \\
    & = \sum_{i=1}^K \beta_i \Big( \sum_s \mu^{\pi_\theta}_{i}(s) b_i (s) \nabla \big( \sum_a \pi (a|s) \big)  \Big) \\
    & = \sum_{i=1}^K \beta_i \Big( \sum_s \mu^{\pi_\theta}_{i}(s) b_i (s) \nabla \big( 1 \big)  \Big) = 0\\
\end{align*}

for any state $s$. The Hessian $\nabla^2_{{\bf w}} \mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}) $ of $\mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w})$ evaluated at ${\bf w}^*$ can be seen to be $ G_{\text{s2r}} (\boldsymbol{\theta})$. The claim follows because $ G_{\text{s2r}} (\boldsymbol{\theta})$ is positive definite for any $\boldsymbol{\theta}$.
\end{proof}

Next, we show that if the parameter is set to be equal to ${\bf w}^*$, then the resulting mean squared error $\mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}^*)$ (now treated as a function of the baselines $b_i(s)$) is further minimized when $b_i(s) = V_i^{\pi_\theta}$. In other words, the variance in the action-value function estimator is minimized if the baseline is chosen to
be the value function itself.


\begin{lemma}
For any given policy $\pi$, the minimum variance baselines $b_i^*(s)$ in the action-value function estimator corresponds to the state-value function $V_i^{\pi_\theta}$.
\end{lemma}

\begin{proof}
For any $d$, let $\mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*)$ denote
\[\mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*) = \sum_{a} \pi(a|s) \frac{1}{2} \big( Q^{\pi_\theta}_i(s,a) - {\bf w}^\top \psi(s,a) - b_i(s) \big)^2 \]
Then $\mathcal{E}^{\pi_\theta}_{\text{s2r}} ({\bf w}^*) = \sum_{i=1}^K \beta_i  \Big( \sum_{s} \mu^{\pi_\theta}_i (s) \mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*) \Big)$. Note that by Assumption \ref{ass:ergodic}, the Markov chain corresponding to any policy $\pi$ is positive recurrent because the number of states is finite. Hence, $ \mu^{\pi_\theta}_i (s) \ge 0$ for all $s \in \mathcal{S}$. Thus, one needs to find the baselines $b_i(s)$ that minimizes $\mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*)$  for each  $s \in \mathcal{S}$. Now for any  $s \in \mathcal{S}$:

\[\frac{\partial \mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*) }{\partial b_i(s)} = - \sum_{a} \pi(a|s) \big( Q^{\pi_\theta}_i(s,a) - {\bf w}^{*\top} \psi(s,a) - b_i(s) \big) \]
For the optimal parameter ${\bf b}_i^*(s)$ we have $\frac{\partial \mathcal{E}^{\pi_\theta, s}_i \big({\bf w}^*, b_i^*(s) \big) }{\partial b_i(s)} = 0$. Then:
\[b_i^*(s) = \sum_{a} \pi(a|s) Q^{\pi_\theta}_i(s,a) - \sum_{a} \pi(a|s) {\bf w}^{*\top}\psi(s,a) \]
The rightmost term equals zero because $\sum_{a} \pi(a|s)\psi(s,a) = 0 $, thus:
\[b_i^*(s) = \sum_{a} \pi(a|s) Q^{\pi_\theta}_i(s,a) =  V^{\pi_\theta}_i(s) \]
The second derivative of $\mathcal{E}^{\pi_\theta, s}_i ({\bf w}^*)$ with respect to $b_i(s)$ is equal to 1. The claim follows.
\end{proof}

From Lemma XXX, ${\bf w}^{*\top} \psi(s,a)$ is a least-squared optimal parametric representation for the action-value functions $Q_i^{\pi_\theta}(s,a)$. On the other hand, from Lemma XXXX, the same is also a least-squared optimal
parametric representation for the advantage functions $A_i^{\pi_\theta}(s,a) = Q_i^{\pi_\theta}(s,a) - V_i^{\pi_\theta}(s) $. The mean squared error XXXX is seen to be minimized w.r.t. the baseline $b_i(s)$ for $b_i(s) = V_i^{\pi_\theta}(s)$, thereby making it more meaningful to consider ${\bf w}^{*\top} \psi(s,a)$ o be the least-squared optimal parametric representation
for the advantage function rather than the action-value function itself.
The temporal difference (TD) error $\delta_i(t)$, for each MDP $M_i$
is a random quantity that is defined according to:
\[\delta_{i,t} = r_{i,t} - \hat{J}_{i,t} + \hat{V}_i \big( s_{i,t+1} \big) - \hat{V}_i \big( s_{i,t} \big)\]
where $\hat{V}_i \big( s_{i,t} \big)$ and $\hat{V}_i \big( s_{i,t+1} \big)$
are unbiased estimate of the differential reward in states $s_{i,t}$ and $s_{i,t+1}$. Likewise, $\hat{J}_{i,t}$ is an unbiased estimate of the average reward from MDP $M_i$. Thus, in particular, these estimates satisfy:
\[\mathbb{E}[\hat{V}_i \big( s_{i,t} \big) | s_{i,t}, \pi_\theta] = V^{\pi_\theta}_i  \big( s_{i,t} \big)\]
\[\mathbb{E}[\hat{J}_{i,t}  | s_{i,t}, \pi_\theta] = J_i  \big( \boldsymbol{\theta} \big)\]
respectively, for any $t > 0$. We assume here that actions are chosen according to policy $\pi_{\theta}$. The next lemma shows that $\delta_{i,t}$
is an unbiased estimate of the advantage function $A_i^{\pi}$.

\begin{lemma}
Under given policy $\pi$ with actions chosen according to it, we have
\[\mathbb{E}[\delta_{i,t} | s_{i,t}, a_{i,t}, \pi] = A_i^{\pi} (s_{i,t} , a_{i,t} )\]
\end{lemma}

\begin{proof}
The proof is according to Lemma 3 in \cite{bhatnagar2008incremental}. Note that:
\begin{align*}
    & \mathbb{E}[\delta_{i,t} | s_{i,t}, a_{i,t}, \pi] = \mathbb{E} \big[ r_{i,t} - \hat{J}_{i,t} + \hat{V}_i \big( s_{i,t+1} \big) - \hat{V}_i \big( s_{i,t} \big) | s_{i,t}, a_{i,t}, \pi \big] \\
    & = r(s_{i,t}, a_{i,t}) - J_i(\pi) + \mathbb{E} \big[ \hat{V}_i \big( s_{i,t+1} \big) | s_{i,t}, a_{i,t}, \pi \big] - V^{\pi}_i  ( s_{i,t} )
\end{align*}
Now
\begin{align*}
    & \mathbb{E} \big[ \hat{V}_i ( s_{i,t+1} ) | s_{i,t}, a_{i,t}, \pi \big] = \mathbb{E} \big[ \mathbb{E} [\hat{V}_i ( s_{i,t+1} ) | s_{i,t+1}, \pi ] \big| s_{i,t}, a_{i,t}, \big] \\
    & = \mathbb{E} \big[ V_i^{\pi} ( s_{i,t+1} ) | s_{i,t}, a_{i,t}, \big] \\
    & = \sum_{s_{i, t+1} \in \mathcal{S}} P_i (s_{i, t+1} | s_{i,t}, a_{i,t}) V_i^{\pi} ( s_{i,t+1} )
\end{align*}

In addition:
\[
r(s_{i,t}, a_{i,t}) - J_i(\pi) + \sum_{s_{i, t+1} \in \mathcal{S}} P_i (s_{i, t+1} | s_{i,t}, a_{i,t}) V_i^{\pi} ( s_{i,t+1} ) = Q^\pi (s_{i,t} , a_{i,t} ) \]
Then:
\[\mathbb{E}[\delta_{i,t} | s_{i,t}, a_{i,t}, \pi] =  Q^\pi (s_{i,t} , a_{i,t} ) - V^{\pi}_i  ( s_{i,t} ) = A^\pi (s_{i,t} , a_{i,t} )\]
\end{proof}

By setting the baselines $b_i(s)$ equal to the value functions $V^{\pi}_i (s)$
The gradient of $J_i(\pi)$ can be written as
\[\nabla J_i (\pi) = \sum_{i=1}^K \beta_i \mathbb{E}_{s \sim \mu^{\pi}_{i}, a \sim \pi} [\psi(s,a) A^{\pi}_i (s,a)] \]
From Lemma XXXX, $\delta_{i,t}$ is an unbiased estimate of the advantage function $A^\pi_i (s_{i,t}, a_{i,t})$. Thus, $\hat \nabla J_i (\pi) = \psi(s_{i,t},a_{i,t}) \delta_{i,t} $ is an unbiased estimate of $\nabla J_i (\pi)$. However, calculating  $\delta_{i,t}$ requires having estimates, $\hat J_i, \hat V_i$, of the average reward and the value function. While
an average reward estimate is simple enough to obtain given the single-stage reward function, the same is not necessarily true for the value function. We use function approximation for the value functions as well. Suppose $\phi(s)$ is a $d$-dimensional feature vector for state $s$. One may then approximate $V_i^\pi(s)$ with ${\bf v}^\top \phi(s)$, where ${\bf v}$ is a
$d$-dimensional weight vector which can be tuned (for a fixed policy $\pi$) using a TD algorithm. In our algorithms, we then use
\[\delta_{i,t} = r_{i,t} - \hat{J}_{i,t} + {\bf v}_t^\top \phi( s_{i,t+1}) - {\bf v}_t^\top \phi( s_{i,t}) \]
as an estimate for the TD error, where ${\bf v}_t$ corresponds to the value function parameter at time $t$. From now on, unless explicitly mentioned, we shall consider $\delta_{i,t}$ to be defined according to XXX. Let $\hat V_i^\pi (s)$ denote the quantity

\[
\hat V_i^\pi (s) = \sum_a \pi(a|s) \big( r(s, a) - J_i(\pi) + \sum_{s' \in \mathcal{S}} P_i (s' | s, a)  {\bf v}^{\pi \top} \phi(s') \big) \]

\subsection{Continuity of eigenvectors}
Let ${\bf x}$ be a left eigenvector of matrix ${\bf P}$ corresponding to eigenvalue $\lambda$, then:
\[{\bf x} {\bf P} = \lambda {\bf x}\]
\[\]

The rank / dimension of ${\bf P - I}$ is $n-1$, meaning we have alinear system with $n-1$ eqautions, since it has an eigenvalue $0$ and it not invertible (there are infinite number of solutions). How ever, if we add the constraint of $\|{\bf x}\|=1$ we add another equation to the system and now we have a single solution. Thus, we can view ${\bf x}$ as a function of ${\bf P}$ and $\lambda$ with only one image to each input. since ${\bf P}$ is continuous 
\[{\bf P} = \beta {\bf P}_1 + (1-\beta)  {\bf P}_2\]
and since $\lambda$ is continuous (Bahita), the ${\bf x}$ is a composition of continuous functions, thus it in continuous. 

Note that the contiouty is on the unit circle, and it is not a straight line. 

==> on_policy_settings.tex <==
{\bf On-policy setting:}
In this setting, the update of the parameters is based on the last observation of the MDP, $\mathcal{O}$. In particular, in Algorithm $\ref{alg:linear_actor_critic}$, the updates are
\[\eta'_{\text{on}} = f_\eta(\eta, \mathcal{O}), \ v'_{\text{on}} = f_v(v, \eta, \mathcal{O}), \ \theta'_{\text{on}} = f_\theta(\theta, \eta, v,  \mathcal{O}).\]
Let $P(X_{\tau+1}|X_\tau) = P_{\text{on}}(X' | X)$ where 
\[P_{\text{on}}(X' | X) \triangleq \begin{cases}
P_{\text{MDP}}(s'| s, a) \cdot \pi_{\theta'_{\text{on}}} (a| s) & \text{if } X = \left[ s, \text{RB} \right] \text{ and } X' = \left[ s', 
     \text{RB} \cup  \mathcal{O} \setminus \text{RB}(\mathcal{O}_{\text{first}}) \right]\\
     0 & \text{Otherwise}
     \end{cases}\]
     
Clearly, $P_{\text{on}}(X' | X)$ depends only on the last observation $X$, therefore  $\{X_\tau\}_{\tau \ge 0}$ with $P_{\text{on}}(X' | X)$ is a Markov process. We can see that the $RB$ information stored at state $X$ is redundant since we don't use it in the selection of the observation that will be used in the parameters update. However we present here this formulation in order to better understand and compare it the other settings. Let's verify that $P_{\text{on}}(X' | X)$ is a row-stochastic matrix:
\begin{align*}
    \sum_{X'} P_{\text{on}}(X' | X) & = \sum_{X'} P_{\text{MDP}}(s'| s, a) \cdot \pi_{\theta'_{\text{on}}} (a| s) \\
    & = \sum_{a} \sum_{s'} P_{\text{MDP}}(s'| s, a) \cdot \pi_{\theta'_{\text{on}}} (a| s) \\
    & = \sum_{a} 1 \cdot \pi_{\theta'_{\text{on}}} (a| s) = 1
\end{align*}
Let's look at the chain:
\begin{align*}
    s_\tau \overbrace{\rightarrow}^{det} \mathcal{O}_{\tau-1} \overbrace{\rightarrow}^{det} \theta_\tau \overbrace{\rightarrow}^{\pi} a_\tau \overbrace{\rightarrow}^{P} s_{\tau+1} \overbrace{\rightarrow}^{det} \mathcal{O}_{\tau} 
    \overbrace{\rightarrow}^{det} \theta_{\tau+1} \overbrace{\rightarrow}^{\pi} a_{\tau+1}
\end{align*}
We can see that $\theta_{\tau+1}$ is based on the last observation $\mathcal{O}_{\tau} = \{s_\tau, a_\tau, r(s_\tau, a_\tau), s_{\tau+1}\}$.


==> rate_of_conv_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rate of Convergence Analysis}

We introduce some notations that will help us in the Lemmas of this section. Let $\{X_t\}_{t \ge 0}$ be a Markov process with transition probability function ${\bf P}_X$. Let $\lambda_1^X, \ldots, \lambda_{|\mathcal{S}|}^X$ be the eigenvalues of ${\bf P}_X$, ordered by $|\lambda_1^X| \ge \ldots |\lambda_{|\mathcal{S}|}^X|$. The matrix ${\bf P}_X$ is a stochastic, hence $\lambda_1^X = 1$. Denote the second largest eigenvalue of ${\bf P}_X$ by $\lambda^X_2$, where $|\lambda^X_2| < 1$. Let $\bar{D}\Big(\lambda_i^X, \epsilon \Big)$
be the closed disk with radius $\epsilon$ and center $\lambda_i^X$. 

We will use the same notations also for these stochastic processes:
$\{Y_t\}_{t \ge 0}$, $\{W_t\}_{t \ge 0}$, $\{Z_t\}_{t \ge 0}$ and $\{U_t\}_{t \ge 0}$. 

Note: Later we will use these notations as follows: \sd{change letter for notations of Markov chains}
\begin{itemize}
    \item $\{X_t\}_{t \ge 0}$ - Real Markov Process.
    \item $\{Y_t\}_{t \ge 0}$ - Sim Markov Process.
    \item $\{W_t\}_{t \ge 0}$ - Slow real Markov Process (by factor $p$).
    \item $\{Z_t\}_{t \ge 0}$ - Real+Sim Markov Process (by interpolation with $\beta$).
    \item $\{U_t\}_{t \ge 0}$ - slow Real + fast Sim Markov Process (by interpolation with $\beta$).
\end{itemize}

\begin{lemma}[Mixing Slow Markov Process with fast Perturbed Markov Process]
\label{lemma:mixing_slow_fast2}
Let $\{X_t\}_{t \ge 0}$ be a Markov process. Let B be a Bernoulli random variable with distribution:
\[\mathbb{P}(B=1)=p\]
\[\mathbb{P}(B=0)=1 - p\]
where $0 \le p \le 1$. Let $\{W_t\}_{t \ge 0}$ be a stochastic process which satisfies:
\begin{align*}
    W_{t+1} = \begin{cases}
    X_{t+1} & \text{if } B=1 \\
    W_t & \text{if } B=0 
    \end{cases}
\end{align*}
where $X_{t+1} \sim {\bf P}_X(X_{t+1}|W_t)$.
We call $\{W_t\}_{t \ge 0}$ a process of slowing $\{X_t\}_{t \ge 0}$ by a factor $p$. 

Let $\{Y_t\}_{t \ge 0}$ be a perturbed Markov process of $\{X_t\}_{t \ge 0}$, such that:
\[\| {\bf P}_X - {\bf P}_Y\| = \epsilon\]

Let  $\{U_t\}_{t \ge 0}$ be a process of mixing $\{W_t\}_{t \ge 0}$ and $\{Y_t\}_{t \ge 0}$ with interpolation coefficient $\beta$, as described in Lemma \ref{lemma:mixing_process}.
Then:
\begin{enumerate}
    \item $\{U_t\}_{t \ge 0}$ is a Markov Process.
    \item Let
    \[\epsilon_1 < \frac{1}{2} \min_{i, j \neq i} |\lambda_{i}^Y - \lambda_{j}^Y|\] 
    where $\lambda_{i}^Y$ and $\lambda_{j}^Y$ are distinct eigenvalue of ${\bf P}_Y$. If ${\bf P}_Y$ is normal matrix and if $\big(p \cdot \epsilon + (1-p) \| {\bf I} - {\bf P}_Y\|  \big) \le \epsilon_1$, then:
    \[d \Big(\sigma({\bf P}_Y), \sigma\big( {\bf P}_U(\beta) \big) \Big)\le \beta \epsilon_1\]
    %\[|\lambda^Y_2 - \lambda^U_2(\beta)| \le \beta \epsilon_1\]
    \item Let
    \[\epsilon_0 < \frac{1}{2} \min_{i,j \neq i} |\lambda_{i}^X - \lambda_{j}^X|\] 
    where $\lambda_{i}^X$ and $\lambda_{i}^X$ are distinct eigenvalue of ${\bf P}_X$. If ${\bf P}_X$ and ${\bf P}_Y$ are normal matrices and if $\epsilon \le \epsilon_0$ and $\big(p \cdot \epsilon + (1-p) \| {\bf I} - {\bf P}_Y\|  \big) \le \epsilon_1$ , then:
    \[d \Big(\sigma({\bf P}_X), \sigma\big( {\bf P}_U(\beta) \big) \Big)\le \epsilon_0 + \beta \epsilon_1\]
    %\[|\lambda^X_2 - \lambda^U_2(\beta)| \le \epsilon_0 + \beta \epsilon_1\]
\end{enumerate}

\end{lemma}

Lemma XXXX shows that the rate of convergence of the combination of "slow real process" and "fast sim process" (process $\{U_t\}_{t \ge 0}$), which follows the mixing sim and real scheme in Algorithm XXXXX, remains in the disk with radios of $\beta \epsilon_1$ compared to sim Markov process. We can see a connection between the the differences in the transition matrix XXXXXX 

==> rate_of_convergence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rate of Convergence Analysis Bounds}
\label{sec:rate_of_convergence_bound}
In this section we sketch an estimate of the convergence rate of the process $Y_\tau$. This convergence rate is intimately related to the second largest  eigenvalue (in absolute value), denoted by $\lambda_2^\theta$, of the induced MC $P^\theta$ \citep{wu2020finite}. We note that a general bound that is based on Assumption  \ref{assumption:sim2real_are_close} and quantifies the distance between the corresponding eigenvalues is still an open question in the context of aperiodic irreducible MCs. Alternatively, we provide a bound based on ergodicity coefficient (EC) that is defined as
$E(P) \triangleq 1 - \min_{i,j}\sum_{s=1}^{|S|}\min(P_{is},P_{js})$. The following lemma bounds $\lambda_2^\theta$. We propose a bound and assert that the bound on $Y_\tau$ convergence-rate is similar as the bound on the real environment.
\begin{lemma}
\label{lemma:ergodicity_coefficient_lemma}
Under Assumption \ref{assumption:sim2real_are_close}, the convergence rate of $Y_\tau$ based on sim and real is worse at most by $|S|\epsilon_{\textrm{s2r}}$.
\end{lemma}
The proof can be found in the supplementary material 
\ref{appendix:rate_of_convergence_bound}.
